Two-loop mixed QCD-EW corrections to $q \overline{q} \to H g$, $qg \to Hq$, and $\overline{q}g \to H\overline{q}$

We compute the two-loop mixed QCD-Electroweak corrections to $q \overline{q} \to H g$ and its crossed channels $q g \to H q$, $\overline{q} g \to H \overline{q}$, limiting ourselves to the contribution of light virtual quarks. We compute the independent helicity amplitudes as well as the form factors for this process, expressing them in terms of hyperlogarithms with algebraic arguments. The Feynman integrals are computed by direct integration over Feynman parameters and the results are expressed in terms of a basis of rational prefactors.

==> scratch.tex <==
The helicity amplitude for $H \to q \overline{q} g$ is divided into two parts, as we did for $\mathcal{A}_\mu$:
\begin{align}
	A_{s_1 s_2 \lambda_3} = A^{\textup{closed}}_{s_1 s_2 \lambda_3} + A^{\textup{open}}_{s_1 s_2 \lambda_3} \,.
\end{align}

The term $A^{\textup{closed}}_{s_1 s_2 \lambda_3}$ does not present any axial component, therefore we can proceed straightforwardly as explained in \cite{Melnikov:2017pgf}. There is only one independent non-zero helicity amplitude. It reads
\begin{align}
	\begin{aligned}
		A^{\textup{closed}}_{-++} = -\iu &\frac{\left( \alpha \alpha_S \right)^{3/2} m_W}{8 \mathrm{\pi} \sin^3 \theta_W} \times	\\
		&\times \frac{1}{2}\left[ 4 + \frac{2}{\cos^4 \theta_W}\left( \frac{5}{4}-\frac{7}{3}\sin^2 \theta_W+\frac{22}{9}\sin^4 \theta_W \right) \right] \frac{s}{\sqrt{2}}\frac{[23]^2}{[12]}F_1^{\textup{closed}}	\,.
	\end{aligned}
\end{align}
The other non-zero helicity can be obtained from the one above using $\mathcal{C}$ and $\mathcal{P}$ invariance:
\begin{align}
	\begin{aligned}
		A^{\textup{closed}}_{+-+}(\mathbf{p}_1,\mathbf{p}_2,\mathbf{p}_3) &= A^{\textup{closed}}_{-++}(\mathbf{p}_2,\mathbf{p}_1,\mathbf{p}_3)	\,,	\\
		A^{\textup{closed}}_{+--}(\mathbf{p}_1,\mathbf{p}_2,\mathbf{p}_3) &= \left( A^{\textup{closed}}_{-++}(\mathbf{p}_1,\mathbf{p}_2,\mathbf{p}_3) \right)^*	\,,	\\
		A^{\textup{closed}}_{-+-}(\mathbf{p}_1,\mathbf{p}_2,\mathbf{p}_3) &= \left( A^{\textup{closed}}_{-++}(\mathbf{p}_2,\mathbf{p}_1,\mathbf{p}_3) \right)^*	\,.
	\end{aligned}
\end{align}
All the other configurations are zero, since QCD interactions do not change the helicity of massless fermions.





~

~

~

~

Once the projector has been absorbed by the polarized external quark $q(\mathbf{p}_1)$, all that remains are QCD interactions: we can therefore apply the same set of relations we used above, as long as we do not alter the chirality of $q(\mathbf{p}_1)$. We get then that
\begin{align}
	\begin{aligned}
		A^{\textup{open},-}_{--\pm}(\mathbf{p}_1,\mathbf{p}_2,\mathbf{p}_3)	&= 0	\,,	\\
		A^{\textup{open},-}_{-+-}(\mathbf{p}_1,\mathbf{p}_2,\mathbf{p}_3)	&= \left( A^{\textup{open},-}_{-++}(\mathbf{p}_2,\mathbf{p}_1,\mathbf{p}_3) \right)^*	\,.
	\end{aligned}
\end{align}

Following the same reasoning, we can write the helicity amplitude
\begin{align}
	\begin{aligned}
		A^{\textup{open},+}_{+--} = -\iu &\frac{\left( \alpha \alpha_S \right)^{3/2} m_W}{8 \mathrm{\pi} \sin^3 \theta_W}\left[ \frac{2}{\cos^4 \theta_W} Q_q^2 \sin^4 \theta_W \right] \frac{s}{\sqrt{2}}\frac{[23]^2}{[12]}F_1^{\textup{open}}	\,,
	\end{aligned}
\end{align}
and the related ones
\begin{align}
	\begin{aligned}
		A^{\textup{open},+}_{++\pm}(\mathbf{p}_1,\mathbf{p}_2,\mathbf{p}_3)	&= 0	\,,	\\
		A^{\textup{open},+}_{+-+}(\mathbf{p}_1,\mathbf{p}_2,\mathbf{p}_3)	&= \left( A^{\textup{open},+}_{+--}(\mathbf{p}_2,\mathbf{p}_1,\mathbf{p}_3) \right)^*	\,.
	\end{aligned}
\end{align}







Relations among different prefactors are obtained analytically, whilst relations among rational monomials are obtained using both analytical and numerical methods, like PSLQ interpolation. All relations are subsequently checked analytically.











\begin{table}[t]
	\centering
	\begin{tabular}{lcccccc}
\toprule
~	&\multicolumn{3}{c}{Rational prefactors $R_j$}	&~&\multicolumn{2}{c}{Rational monomials $M_k$}	\\
~						&Original	&Partial reduction &Basis		&~&Partial reduction	&Basis	\\
\midrule
\multirow{2}*{$F^{\textup{closed}}$}		&46 (45)	&???	&???	&~	&45		&???	\\
											&46 (45)	&22		&15		&~	&???	&28		\\%[2em]
\multirow{2}*{$F^{\textup{open},N_c}$}		&1410	&234	&200?	&~	&1454	&???	\\
											&1413	&213	&193?	&~	&1389	&1276?	\\%[2em]
\multirow{2}*{$F^{\textup{open},1/N_c}$}	&5526	&???	&???	&~	&???	&???	\\
											&???	&???	&???	&~	&???	&???	\\
\midrule
\multirow{2}*{$A_{\textup{LO},\epsilon^0}$}	&19~(40)    &11~(40)    &???	&~	&40		&???	\\
											&18~(37) 	&11~(37)	&11		&~	&???	&33		\\%[2em]
\multirow{2}*{$A_{\textup{LO},\epsilon^1}$}	&63		&???	&???	&~	&151	&???	\\
											&???	&39		&26		&~	&???	&94		\\%[2em]
\multirow{2}*{$A_{\textup{LO},\epsilon^2}$}	&145	&???	&???	&~	&218	&???	\\
											&???	&53		&39		&~	&???	&188	\\
\bottomrule
	\end{tabular}
	\caption{Number of linearly-independent rational prefactors and rational monomials at different stages of the reduction procedure. For comparison, we list first the different component $F$ of the two-loop NLO amplitude and then the first three non-zero orders $A_{\textup{LO}}$ in the $\epsilon$ for the LO amplitude.}
	\label{NumPref}
\end{table}








We provide the expression of the renormalized finite remainder of the amplitude in terms of the unrenormalized quantities in Appendix~\ref{sec:finrem}, and its expression in terms of GPLs and rational prefactors in the ancillary files.









~

The axial term may be non-vanishing in the case of diagrams where both of the EW boson are attached to the external quark line. It is possible to bypass the direct computation of expressions containing $\gamma_5$ by considering polarized external states: by anticommuting $\gamma_5$ until it touches the spinor $\overline{u}_{L/R}(\mathbf{p}_1)$, such a matrix coming from the EW vertices is absorbed into the left- or right-chirality projectors $\mathbb{P}_{L} = \frac{1-\gamma_5}{2}$ and $\mathbb{P}_{R} = \frac{1+\gamma_5}{2}$, respectively. The resulting expression does not contain axial terms anymore and can be computed using the same procedure as for $\mathcal{A}^{\textup{closed}}_\mu$, with an overall coefficient determined by the type and chirality of the quark $q(\mathbf{p}_1)$. Specifically, for $\overline{u}_{L}(\mathbf{p}_1) = \overline{u}(\mathbf{p}_1) \mathbb{P}_L$ we obtain
%\todo{L: Are the colors put on purpose here? It looks a bit too much to me}\Marco{Up to you to choose between the $\textcolor{blue}{\pm}$ and the $\textcolor{orange}{L/R}$ notation. I will remove the other and fix the colors.}
\begin{align}
	\label{AopenP}
%	\begin{aligned}
%		\mathcal{A}^{\textup{open},\textcolor{blue}{+}\textcolor{orange}{L}}_\mu = -\iu &\frac{\left( \alpha \alpha_S \right)^{3/2} m_W}{8 \mathrm{\pi} \sin^3 \theta_W}\left[ \frac{2}{\cos^4 \theta_W} Q_q^2 \sin^4 \theta_W \right]	\\
%		&\times \mathbb{P}_L \left[ \left( \slashed{p}_3 p_{2\mu} - p_2 \cdot p_3 \gamma_\mu \right) F_1^{\textup{open}} + \left( \slashed{p}_3 p_{1\mu} - p_1 \cdot p_3 \gamma_\mu \right) F_2^{\textup{open}} \right]	, 
%	\end{aligned}\\
    \begin{aligned}
		\mathcal{A}^{\textup{open},L}_\mu = - &\textcolor{blue}{\iu}\frac{\alpha^{3/2} \alpha_S^{1/2} m_W}{2 \sin^3 \theta_W}\left( \frac{2}{\cos^4 \theta_W} Q_q^2 \sin^4 \theta_W \right) \mathbb{P}_L \left[ \tau_{1,\mu} F_{1,m_Z}^{\textup{open}} + \tau_{2,\mu} F_{2,m_Z}^{\textup{open}} \right]	, 
	\end{aligned}
\end{align}
while for $\overline{u}_{R}(\mathbf{p}_1) = \overline{u}(\mathbf{p}_1) \mathbb{P}_R$ we get
\begin{align}
	\label{AopenM}
%	\begin{aligned}
%		\mathcal{A}^{\textup{open},\textcolor{blue}{-}\textcolor{orange}{R}}_\mu = -\iu &\frac{\left( \alpha \alpha_S \right)^{3/2} m_W}{8 \mathrm{\pi} \sin^3 \theta_W}\left[ 1 + \frac{2}{\cos^4 \theta_W}\left( T_q - Q_q \sin^2 \theta_W \right)^2 \right]	\\
%		&\times \mathbb{P}_R \left[ \left( \slashed{p}_3 p_{2\mu} - p_2 \cdot p_3 \gamma_\mu \right) F_1^{\textup{open}} + \left( \slashed{p}_3 p_{1\mu} - p_1 \cdot p_3 \gamma_\mu \right) F_2^{\textup{open}} \right]	,
%	\end{aligned}
%	\begin{aligned}
%		\mathcal{A}^{\textup{open},R}_\mu = - &\frac{\mathrm{\pi}^2 \alpha^{3/2} \alpha_S^{1/2} m_W}{2 \sin^3 \theta_W}\left[ 1 + \frac{2}{\cos^4 \theta_W}\left( T_q - Q_q \sin^2 \theta_W \right)^2 \right]	\\
%		&\times \mathbb{P}_R \left[ \left( \slashed{p}_3 p_{2\mu} - p_2 \cdot p_3 \gamma_\mu \right) F_1^{\textup{open}} + \left( \slashed{p}_3 p_{1\mu} - p_1 \cdot p_3 \gamma_\mu \right) F_2^{\textup{open}} \right]	,
%	\end{aligned}   \\
	\begin{aligned}
		\mathcal{A}^{\textup{open},R}_\mu = - &\textcolor{blue}{\iu}\frac{\alpha^{3/2} \alpha_S^{1/2} m_W}{2 \sin^3 \theta_W}\left\{\mathbb{P}_R \left[ \tau_{1,\mu} F_{1,m_W}^{\textup{open}} + \tau_{2,\mu} F_{2,m_W}^{\textup{open}} \right] + \right.\\
		&\left.+ \frac{2}{\cos^4 \theta_W}\left( T_q - Q_q \sin^2 \theta_W \right)^2 \mathbb{P}_R \left[ \tau_{1,\mu} F_{1,m_Z}^{\textup{open}} + \tau_{2,\mu} F_{2,m_Z}^{\textup{open}} \right]\right\}	,
	\end{aligned}
\end{align}
where  $Q_q$ and $T_q$ are the electric charge of the quark $q(\mathbf{p}_1)$ and its eigenvalue of the third generator of $\mathrm{SU}(2)_L$, respectively (see e.g.\ \cite{Romao:2012pq}). We assume the Cabibbo--Kobayashi--Maskawa mixing matrix to be the identity matrix.\footnote{This approximation is justified because the off-diagonal entries are strongly suppressed.} $\mathcal{A}^{\textup{open},L}_\mu$ receives contributions only from the $Z$ boson, while $\mathcal{A}^{\textup{open},R}_\mu$ is sensitive to the $W$ boson as well.









\begin{table}[t]
	\centering
    \small
	\begin{tabular}{lccccc}
\toprule
~       &Original	&{Partial reduction} &{Monomial reduction}  &{Basis}		&{No zeroes}	\\
\midrule
\multirow{2}*{$\tilde{F}_{\epsilon^0}^{\textup{closed}}$}		&46~(45)	&22~(45)	&22~(28)	&15~(28)	&10~(17)	\\
											&46~(45)    &22~(45)	&22~(28)	&15~(28)	&10~(17)    \\
\multirow{2}*{$\tilde{F}_{\epsilon^0}^{N_c}$}		&1410~(1454)    &234~(1294)	&234~(1093)	&134~(1093)	&100~(983)    \\
											&1413~(1389)	&213~(1285)	&213~(1186)	&134~(1186)	&117~(1169)    \\
\multirow{2}*{$\tilde{F}_{\epsilon^0}^{1/N_c}$}	&5526~(6789)	&1174~(6788)	&1100~(5177)    &690~(3823)	&325~(983)    \\
											&5524~(5905)	&1139~(5894)    &1139~(4604)    &784~(4517)	&460~(1169)    \\
\midrule
\multirow{2}*{$\tilde{F}_{\epsilon^0}^{\textup{open},(1)}$}	&19~(40)    &11~(40)    &11~(35)    &11~(35)    &8~(25)	\\
											&18~(37) 	&11~(37)	&11~(33)	&11~(33)	&8~(21)    \\
\multirow{2}*{$\tilde{F}_{\epsilon^1}^{\textup{open},(1)}$}	&63~(151)	&39~(151)	&39~(95)	&26~(95)	&14~(32)	\\
											&62~(139)	&36~(139)	&36~(110)	&26~(110)	&17~(45)	\\
\multirow{2}*{$\tilde{F}_{\epsilon^2}^{\textup{open},(1)}$}	&160~(244)	&58~(244)	&58~(197)	&39~(197)	&15~(45)	\\
											&157~(232)	&55~(232)	&55~(169)	&39~(169)	&14~(27)    \\
\bottomrule
	\end{tabular}
	\caption{Number of linearly-independent rational prefactors (and rational monomials) at different stages of the reduction procedure. For comparison, we list first the different component $F$ of the two-loop NLO amplitude and then the first three non-zero orders $A_{\textup{LO}}$ in the $\epsilon$ expansion for the LO amplitude. The two rows of each terms report about the content of first and second form factor.}
	\label{NumPrefOLD}
\end{table}







\begin{table}[t]
	\centering
    \small
	\begin{tabular}{lcccS}
\toprule
~       &{Rational prefactors}	&{Transcendental terms} 	&{Maximum weight} &{Final size ($\unit{\kibi\byte}$)} \\
\midrule
\multirow{2}*{$\tilde{F}_{\epsilon^0}^{\textup{closed}}$}		&10~(17)	&10~(407)	&4    &46.9    \\
											&10~(17)	&10~(407)	&4    &46.9    \\
\multirow{2}*{$\tilde{F}_{\epsilon^0}^{N_c}$}		&30~(98)	&30~(9979)	&4    &10035.7    \\
											&30~(184)	&30~(10\,048)	&4    &10110.9    \\
\multirow{2}*{$\tilde{F}_{\epsilon^0}^{1/N_c}$}	&54~(151)	&54~(25\,239)	&4    &15962.6    \\
											&82~(592)	&82~(24\,349)	&4    &11268.1    \\
\midrule
\multirow{2}*{$\tilde{F}_{\epsilon^0}^{\textup{open},(1)}$}	&4~(11)	    &4~(19)	    &2    &1.3    \\
											&4~(9)	    &4~(13)	    &2    &0.9    \\
\multirow{2}*{$\tilde{F}_{\epsilon^1}^{\textup{open},(1)}$}	&7~(15) 	&7~(114)	&3    &7.0    \\
											&7~(32)	    &7~(138)	&3    &9.0    \\
\multirow{2}*{$\tilde{F}_{\epsilon^2}^{\textup{open},(1)}$}	&10~(36)	&10~(942)	&4    &192.5    \\
											&9~(11)	    &9~(978)	&4    &153.1    \\
\bottomrule
	\end{tabular}
	\caption{Final number of rational prefactors and transcendental terms, with the number of "monomial" components indicated between brackets.}
	\label{IterPrefOLD}
\end{table}



\begin{table}[t]
	\centering
    \small
	\begin{tabular}{lrlrlrl}
\toprule
~       &\multicolumn{2}{c}{$P_{q\overline{q}}$}	&\multicolumn{2}{c}{$P_{qg}$} 	&\multicolumn{2}{c}{$P_{\overline{q}g}$} \\
\midrule
$\tilde{F}_{\epsilon^0}^{\textup{open},(1)}$ &&$+0.33015\,\iu$	         &$-0.56738$&$+0.07938\,\iu$	    &$-0.56797$&$-0.20133\,\iu$    \\
\midrule
$\tilde{F}_{\textup{fin}}^{\textup{closed}}$ &$-0.23290$&$-0.43682\,\iu$ &$+1.03532$&$+0.01177\,\iu$	 &$1.7070$&$+0.0218\,\iu$    \\
$\tilde{F}_{\textup{fin}}^{N_c}$		     &$+0.76270$&$+0.00387\,\iu$ &$-0.58966$&$-1.61547\,\iu$	 &$-0.827337$&$-3.71626\,\iu$    \\
$\tilde{F}_{\textup{fin}}^{1/N_c}$         	 &$-34.7761$&$-268.082\,\iu$ &$1247.76$&$-375.259\,\iu$	 &$428.401$&$-728.775\,\iu$    \\
$\tilde{F}_{\textup{fin}}^{N_f}$	         &$+0.04632$&	             &$0.320341$&$+0.124712\,\iu$ &$0.224783$&$+0.310246\,\iu$    \\
\bottomrule
	\end{tabular}
	\caption{Numerical values of the different parts of the LO and NLO form factors, evaluated at points defined in Eq.~\eqref{pointstable}.}
\end{table}










\begin{table}[t]
	\centering
    \small
	\begin{tabular}{lccc}
\toprule
~       &$P_{q\overline{q}}$	&$P_{qg}$ 	&$P_{\overline{q}g}$ \\
\midrule
$\tilde{F}_{\epsilon^0}^{\textup{open},(1)}$ &$0.33015\,\iu$	                  &$-0.56738+0.07938\,\iu$	    &$-0.56797-0.20133\,\iu$    \\
\midrule
$\tilde{F}_{\textup{fin}}^{\textup{closed}}$ &$-0.23290-0.43682\,\iu$	  &$1.03532+0.01177\,\iu$	 &$1.7070+0.0218\,\iu$    \\
$\tilde{F}_{\textup{fin}}^{N_c}$		     &$ 0.76269+0.0038708\,\iu$ &$-0.589663-1.61547\,\iu$	 &$-0.827337-3.71626\,\iu$    \\
$\tilde{F}_{\textup{fin}}^{1/N_c}$         	 &$-34.7761-268.082\,\iu$	  &$1247.76-375.259\,\iu$	 &$428.401-728.775\,\iu$    \\
$\tilde{F}_{\textup{fin}}^{N_f}$	         &$0.0463183$	              &$0.320341+0.124712\,\iu$ &$0.224783+0.310246\,\iu$    \\
\bottomrule
	\end{tabular}
	\caption{Numerical values of the different parts of the LO and NLO form factors, evaluated at points defined in Eq.~\eqref{pointstable}.}
	\label{numerics}
\end{table}








\begin{table}[t]
	\centering
    \small
	\begin{tabular}{cSSSS}
\toprule
~                           &{Addends}  &{Transcendental terms} &{Weight}           &{Size ($\unit{\kibi\byte}$)} \\
\midrule
$\tilde{A}_{\epsilon^0}$    &4	        &16	                    &\SIrange{1}{2}{}   &    0.9 \\
%$\tilde{F}_{2,\epsilon^0}^{\textup{open},(1)}$  &4          &22	                    &\SIrange{1}{2}{}   &    1.0 \\
$\tilde{A}_{\epsilon^1}$    &7 	        &100	                &\SIrange{1}{3}{}   &    5.6 \\
%$\tilde{F}_{2,\epsilon^1}^{\textup{open},(1)}$  &7	        &104	                &\SIrange{1}{3}{}   &    5.7 \\
$\tilde{A}_{\epsilon^2}$    &9	        &449	                &\SIrange{1}{4}{}   &   34.1 \\
%$\tilde{F}_{2,\epsilon^2}^{\textup{open},(1)}$  &9	        &457	                &\SIrange{1}{4}{}   &   30.3 \\
\midrule
$\tilde{B}_{1}$             &4	        &32                     &\SIrange{2}{3}{}   &    3.1 \\
%$\tilde{B}_{2}$             &4	        &44                     &\SIrange{2}{3}{}   &    2.9 \\
$\tilde{C}_{1}$             &30	        &10089                  &\SIrange{1}{4}{}   & 4614.1 \\
%$\tilde{C}_{2}$             &30	        &10151	                &\SIrange{1}{4}{}   & 4925.8 \\
$\tilde{D}_{1}$             &54 	    &25332                  &\SIrange{1}{4}{}   & 9355.7 \\
%$\tilde{D}_{1}$             &54	        &24450	                &\SIrange{1}{4}{}   & 9355.8 \\
$\tilde{E}_{1}$             &54 	    &25332                  &\SIrange{1}{4}{}   &   41.4 \\
\bottomrule
	\end{tabular}
	\caption{Final number of rational prefactors and transcendental terms, without taking into account the part proportional to $\log(m_V^2/\mu^2)$ in the finite remainder.}
	\label{IterPref}
\end{table}
%\midrule
%$\tilde{E}_{1}$             &10         &407                    &\SIrange{1}{4}{}   &   41.4 \\
%$\tilde{E}_{2}$             &10         &407                    &\SIrange{1}{4}{}   &   41.4 \\
%$\tilde{F}_{1,\epsilon^0}^{N_c}$ &30    &9979	                &\SIrange{1}{4}{}   & 9070.7 \\
%$\tilde{F}_{2,\epsilon^0}^{N_c}$ &30    &10048                  &\SIrange{1}{4}{}   & 9176.2 \\
%$\tilde{F}_{1,\epsilon^0}^{1/N_c}$ &54	&25239	                &\SIrange{1}{4}{}   &14711.2 \\
%$\tilde{F}_{2,\epsilon^0}^{1/N_c}$ &82	&24349	                &\SIrange{1}{4}{}    &10348.5 \\




\begin{table}[t]
	\centering
    \small
	\begin{tabular}{cSSSr}
\toprule
~                           &{Addends}  &{Transcendental terms} &{Weight}           &\multicolumn{1}{c}{Size} \\
\midrule
$\tilde{A}_{\epsilon^0}$    &4	        &16	                    &\SIrange{1}{2}{}   &    \SI{0.9}{\kibi\byte} \\
$\tilde{A}_{\epsilon^1}$    &7 	        &100	                &\SIrange{1}{3}{}   &    \SI{5.6}{\kibi\byte} \\
$\tilde{A}_{\epsilon^2}$    &9	        &449	                &\SIrange{1}{4}{}   &    \SI{34.1}{\kibi\byte} \\
\midrule
$\tilde{B}_{1}$             &4	        &32                     &\SIrange{2}{3}{}   &    \SI{2.9}{\kibi\byte} \\
$\tilde{C}_{1}$             &30	        &10089                  &\SIrange{1}{4}{}   &    \SI{4.6}{\mebi\byte} \\
$\tilde{D}_{1}$             & 	    &                  &\SIrange{1}{4}{}   &\SI{1.3}{\mebi\byte}  \\
$\tilde{E}_{1}$             &~ 	        &~                      &\SIrange{1}{4}{}   &   \SI{62.0}{\kibi\byte} \\
\bottomrule
	\end{tabular}
	\caption{Final number of rational prefactors and transcendental terms for the first form factor, without taking into account the part proportional to $\log(m_V^2/\mu_R^2)$ in the finite remainder.}
	\label{IterPref}
\end{table}

